Privacy-Preserving Financial Anomaly Detection via Federated Learning & Multi-Party Computation

One of the main goals of financial institutions (FIs) today is combating fraud and financial crime. To this end, FIs use sophisticated machine-learning models trained using data collected from their customers. The output of machine learning models may be manually reviewed for critical use cases, e.g., determining the likelihood of a transaction being anomalous and the subsequent course of action. While advanced machine learning models greatly aid an FI in anomaly detection, model performance could be significantly improved using additional customer data from other FIs. In practice, however, an FI may not have appropriate consent from customers to share their data with other FIs. Additionally, data privacy regulations may prohibit FIs from sharing clients' sensitive data in certain geographies. Combining customer data to jointly train highly accurate anomaly detection models is therefore challenging for FIs in operational settings. In this paper, we describe a privacy-preserving framework that allows FIs to jointly train highly accurate anomaly detection models. The framework combines the concept of federated learning with efficient multi-party computation and noisy aggregates inspired by differential privacy. The presented framework was submitted as a winning entry to the financial crime detection track of the US/UK PETs Challenge. The challenge considered an architecture where banks hold customer data and execute transactions through a central network. We show that our solution enables the network to train a highly accurate anomaly detection model while preserving privacy of customer data. Experimental results demonstrate that use of additional customer data using the proposed approach results in improvement of our anomaly detection model's AUPRC from 0.6 to 0.7. We discuss how our framework, can be generalized to other similar scenarios.

==> teamintro.tex <==
\section{Team Introduction}

%\panos{Briefly introduce yourself and/or the members of your time. Include your background and expertise. Optionally, explain your interest in the problem and competition.
%}

Our team is comprised of members of Visa Research, with background in cryptography, security, privacy enhancing technologies, blockchain, secure computation, machine learning, and deep learning. Visa and, by extension, our Visa Research team, has a special interest in payment fraud detection; we feel committed to treating data with care and exploring privacy-preserving settings.


